Network Science, Homophily and Who Reviews Who in the Linux Kernel?

In this research, we investigate peer review in the development of Linux by drawing on network theory and network analysis. We frame an analytical model which integrates the sociological principle of homophily (i.e., the relational tendency of individuals to establish relationships with similar others) with prior research on peer-review in general and open-source software in particular. We found a relatively strong homophily tendency for maintainers to review other maintainers, but a comparable tendency is surprisingly absent regarding developers' organizational affiliation. Such results mirror the documented norms, beliefs, values, processes, policies, and social hierarchies that characterize the Linux kernel development. Our results underline the power of generative mechanisms from network theory to explain the evolution of peer review networks. Regarding practitioners' concern over the Linux commercialization trend, no relational bias in peer review was found albeit the increasing involvement of firms.

==> bibliographies.config.tex <==

%

\RequirePackage{etoolbox}

\newtoggle{bibtex_natbib}
%
\settoggle{bibtex_natbib}{false}

%

\newtoggle{biber_biblatex}
\settoggle{biber_biblatex}{true}
%


%


%


%

\iftoggle{bibtex_natbib}{
  \typeout{On bibtex_natbib mode for bibliographies}
}{} 


\iftoggle{biber_biblatex}{
  \typeout{On biber_biblatex mode for bibliographies}
}{} 


%
\iftoggle{bibtex_natbib}{
  \iftoggle{biber_biblatex}{
    \typeout{ERROR: Chose among packages and pre-processors of bibliographies}
    \typeout{Either bibtex_natbib or biber_biblatex}
    \stop}{} 
}{} 


%

\iftoggle{bibtex_natbib}{
}{ \iftoggle{biber_biblatex}{}
  {
    \typeout{ERROR: Chose one package and pre-processor of bibliographies}
    \typeout{Either bibtex_natbib or biber_biblatex}
    \stop
  }
} 








==> latextoolsforwritingacademicpapers/reviewAndCommentTools.tex <==
%
%
%

%


\usepackage{xargs} 
%
\RequirePackage[usenames,dvipsnames]{xcolor}
\usepackage{stackengine}

%
%
%
%
\RequirePackage[disable,colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}

%


%

%


%
%
%
%
%

%

\newcommandx{\error}[2][1=]{\todo[linecolor=red,backgroundcolor=red!50,bordercolor=red,#1]{#2}}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}

%
%

%
%


%

%

%
\newenvironment{drafte} {\color{violet}}

%

%
   
%
\newcommand{\draftp}[1]{\textcolor{violet}{#1}}  

%


%

%

\setstackgap{L}{.5\baselineskip}
\newcommand\markabove[2]{{\sffamily\color{red}\hsmash{$\uparrow$}%
  \smash{\toplap{#1}{\scriptsize\bfseries#2}}}}
\newcommand\markbelow[2]{{\sffamily\color{red}\hsmash{$\downarrow$}%
  \smash{\bottomlap{#1}{\scriptsize\bfseries#2}}}}
  
%
%
%
%



%


%
\newcommand{\boxreview}[2]{\parbox{\linewidth}{
\vspace{0.2cm}
\scriptsize\bfseries\sffamily\color{red}{#1} commented -- {#2}}
\vspace{0.2cm}
}  

%

%




   
%
\newcommand{\newPara}[1]{\textcolor{Sepia}{#1}}  



\newenvironment{newStuff}%
%
%
%
{
    \begin{color}{Sepia}
    \begin{tabular}{|p{1.0\textwidth}|}
    \hline\\
    }
    { 
    \\\\\hline
    \end{tabular} 
    \end{color}
    }


==> wp-template.config.tex <==
\RequirePackage{etoolbox}

\RequirePackage[usenames,dvipsnames]{xcolor}


\definecolor{bmcblue}{rgb}{0,0.2,0.4}
\definecolor{joseViolet2016}{rgb}{0.44,0.16,0.39}


\definecolor{docheadcolor}{rgb}{0.44,0.16,0.39}

